Blockchain Meets Database: Design and Implementation of a Blockchain Relational Database

In this paper, we design and implement the first-ever decentralized replicated relational database with blockchain properties that we term blockchain relational database. We highlight several similarities between features provided by blockchain platforms and a replicated relational database, although they are conceptually different, primarily in their trust model. Motivated by this, we leverage the rich features, decades of research and optimization, and available tooling in relational databases to build a blockchain relational database. We consider a permissioned blockchain model of known, but mutually distrustful organizations each operating their own database instance that are replicas of one another. The replicas execute transactions independently and engage in decentralized consensus to determine the commit order for transactions. We design two approaches, the first where the commit order for transactions is agreed upon prior to executing them, and the second where transactions are executed without prior knowledge of the commit order while the ordering happens in parallel. We leverage serializable snapshot isolation (SSI) to guarantee that the replicas across nodes remain consistent and respect the ordering determined by consensus, and devise a new variant of SSI based on block height for the latter approach. We implement our system on PostgreSQL and present detailed performance experiments analyzing both approaches.

==> related_work.tex <==
\vspace{-.2cm}
\section{Related Work}
\label{sec:related}
\textbf{Bitcoin}~\cite{bitcoin} and \textbf{Ethereum}~\cite{ethereum}
adopt an order-execute model, where transactions are first ordered in a block through consensus
(such as proof-of-work) and each node validates and commits transactions to its copy of the blockchain
by serially executing each transaction. In our \textit{order-execute} approach, we leverage SSI %available in databases 
to execute transactions concurrently. Further, such platforms only support
a simple key-value data model. % with no support for rich queries or provenance queries.

\textbf{Hyperledger Fabric}~\cite{fabric} adopts an \textit{execute-then-order} approach, where transactions are first
executed and endorsed by multiple nodes, then ordered by consensus, and then followed by serial validation and commit.
In contrast, in our \textit{execute-order-in-parallel} approach transaction execution and ordering happen parallelly. %,
%with no need for a client to collect endorsements from multiple peers. 
Fabric only supports leveldb and couchdb as the underlying database, with support for composite keys and range queries. %Richer queries in
%couchdb are permitted only for read-only queries as it could result in phantom reads. 
In contrast, we support the full spectrum of
SQL queries in a smart contract (for the first time) with the exception of libraries that could introduce non-determinism and
blind updates. Further, by leveraging capabilities already available within a relational database we provide support
for complex data types, schemas, constraints, and provenance queries. Performance studies on Fabric~\cite{fabric, perfFabric1}
have shown that a throughput of 3000 tps can be achieved with goLevelDB as the state database for a
\texttt{simple} smart-contract, while the throughput drops to 700 tps with CouchDB.
\par
\textbf{Hyperledger Composer}~\cite{composer} is a set of collaboration tools for building blockchain business networks utilizing
Hyperledger Fabric. It allows a user to write a basic SQL query with limited syntax~\cite{composer-query}
and internally converts the SQL query to a JSON selector query~\cite{couchdb-query} supported by CouchDB.
		%, and make it significantly simpler to implement
%checkpoint-recovery. SENTHI: this is significantly different from what a blockchain needs
%Our \textit{execute-order-in-parallel} approach is closest in design to Hyperledger Fabric~\cite{fabric},
%where transactions are first executed concurrently by endorser nodes, who sign the read and write sets obtained from execution
%and return them to the client (referred to as endorsement phase).
%If multiple endorser nodes produce the same read-write sets, the client submits the transaction to an ordering service,
%which orders transactions into blocks. Each node then sequentially
%performs a MVCC check on the read-write sets of each transaction to determine which ones are valid and can commit.
%While the separation of transaction execution and ordering and the notion of a pluggable ordering service are similar
%in our design with Fabric, there are several key differences. First, in Fabric the endorsement phase must complete before
%the transaction can be submitted to the ordering service to be ordered. In contrast, we remove the need for a client to collect
%endorsements, permitting the execution of transactions to happen in parallel with ordering. Our novel SSI based on block height
%ensures a serializable ordering of transactions among all peers and maintains the replicas in a consistent state. Second, 

%In both our system and in Fabric, no two transactions within the same block can modify the same version of a particular
%state (a key or a row), as it would result in a MVCC error. However, in Ethereum, given its sequential execution of transactions
%post ordering, it is possible to commit two transactions in the same block that modify the same state variable, as the second
%transaction can read the update made by the first transaction.

\textbf{Corda}~\cite{corda} refers to their platform as a decentralized database. % primarily targeting financial services use cases.
%They adopt a UTXO model, where states are objects typically representing financial assets that are owned by users
%in the system. Transactions involve spending states and creating new versions of the state, that are marked as unspent.
Transactions are executed by one node at a time (not parallelly executed by all nodes) and the results are shared with other 
nodes that have a need to know. %, along with the entire dependency graph of historical transactions that modified this state. 
%Flows in Corda
%automate the process of validating the historical transactions to ensure that there is no double spending, i.e., no two
%transactions modify the same unspent state. 
There is no notion of a blockchain in Corda. However, optionally, a notary
could order transactions and validate them for double spending. %, which it does based on a timestamp (the transaction arriving later that tries
%to modify a state that is already spent is invalidated). 
Corda uses the H2 embedded SQL engine as the state database. State objects can define a relational mapping, and an
object serialization framework is used to store the states in a relational database. This permits querying the
database using SQL and also permits rich queries (such as joins) with an organization's private non-blockchain data.
However, it does not enable rich query support within the smart contract itself.

\textbf{Veritas}~\cite{veritas} proposes shared verifiable tables %and implemented a prototype 
using a set of Redis key-value stores each owned by an organization.
Only the verifiability property, i.e., immutable logs, is supported. For ensuring consistency across replicas,
it uses a centralized trusted timestamp server to order transactions. Further, a transaction
is executed only on one of the nodes, and each node periodically ships logs of multiple read-write sets
to other nodes via a Kafka-based broadcast service. Nodes are trusted to execute and share results
correctly with other nodes, and hence is not decentralized. Nodes vote on transactions to resolve
any conflicts.
%As a result, this approach trust the
%transaction execution results of other nodes and hence, not decentralized. On receiving a
%logs of read-write sets, each node
%validates the log along with the locally maintained log for conflicts (as each node would have
%executed different transactions) to perform voting on transactions. Similar to blockchain
%and non-blockchain schema that we proposed, this work supports shared and private tables.

\textbf{BigchainDB}~\cite{bigchaindb} employs Tendermint consensus~\cite{tendermint, tendermint-url} over a set
of independent MongoDB~\cite{mongodb} instances, %a document store, 
each owned by a different organization. It supports immutability and decentralization. While the overall
goals of BigchainDB are similar to ours, there are fundamental architectural differences. It supports
only user tokens/assets similar to Bitcoin
and no support for smart contracts. A transaction submitted to BigchainDB is forwarded to
Tendermint nodes, which %takes care of proposing new blocks and making 
ensure that all the BigchainDB nodes
agree on the next block in a Byzantine fault tolerant way. %Each BigchainDB node keeps track of
%the block-under-construction by collecting the transactions delivered (by \texttt{DeliverTx}) between the
%\texttt{BeginBlock} and \texttt{EndBlock} calls. When the Tendermint finally issues a \texttt{Commit},
%all transactions are executed serially and committed. 
Transactions are serially executed post ordering, similar to Ethereum.

It is evident from the related work that ours is the first blockchain relational database
with rich features of both blockchain and databases. Further, the \textit{execute-and-order-in-parallel}
approach proposed in this paper is highly novel and we believe it is applicable to
centralized replicated databases.

